A remark on higher order RUE-resolution with EXTRUE

We show that a prominent counterexample for the completeness of first order RUE-resolution does not apply to the higher order RUE-resolution approach EXTRUE.

==> seki-deckblatt.tex <==
% This file must not be modified!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
\typeout{CP's SEKI-deckblatt, Version 2.18, 24/11/2004 15.00 h}

\catcode`\@=11

\newcommand\SEKIREPORTTYPE
{\ifcase\SEKITYPE SEKI Report\or SEKI Working Paper\or Internet Copy\fi}

\newcommand\makecover{{%
  \def\majorfootroom{\raisebox{-1.9ex}{\rule{0ex}{.5ex}}}
  \def\footroom{\raisebox{-1.5ex}{\rule{0ex}{.5ex}}}
\ifcase\SEKITYPE
  \def\WHATAMI{{\large\SEKIREPORTTYPE\ SR--\SEKIYEAR--\SEKINUMBEROFYEAR}}
  \def\Titlepagetype{{\GIGA SEKI\sf\huge-REPORT ISSN 1437-4447}}
\or             
  \def\WHATAMI{{\large\SEKIREPORTTYPE\ SWP--\SEKIYEAR--\SEKINUMBEROFYEAR}}
  \def\Titlepagetype{{\GIGA SEKI\sf\Huge-WORKING-PAPER}}
\or
  \def\WHATAMI{{\large\SEKIREPORTTYPE: May 1, 2006}}
  \def\Titlepagetype{{\GIGA OMEGA \sf\huge PUBLICATION}}
\fi
\setcounter{page}{-99}%
\thispagestyle{empty}%
\mbox{}\vspace{8cm}\vfill\par\mbox{}\hfill\robbiuni
\vspace{1cm}\par\mbox{}\hfill
\def\fboxrule{2mm}%
\framebox{\raisebox{-2.9cm}{\rule{0ex}{5.8cm}}\begin{minipage}{10.4cm}
\begin{center}
\large\bf\@title\majorfootroom\mbox{}\vfill\par
\rm\normalsize\def\thanks##1{}\@author\majorfootroom\mbox{}\vfill\par
\WHATAMI
\vskip-.5ex\vfill
\end{center}
\end{minipage}}
\vskip-22.3cm
\noindent
\begin{sideways}
\begin{minipage}{22cm}
\sf\Titlepagetype\hfill
\begin{tabular}[c]{l}
  UNIVERSIT\"AT DES SAARLANDES
\\FACHRICHTUNG INFORMATIK
\\D--66123 SAARBR\"UCKEN
\\GERMANY
\\{\scriptsize WWW: \texttt{http://www.ags.uni-sb.de/}}
\\\mbox{}
\\\end{tabular}
\end{minipage}
\end{sideways}
\newpage
\mbox{}
\vfill
\par\noindent
\ifcase\SEKIPUBLISHEDTYPE
\or
  {\bf This \SEKIREPORTTYPE\ is published as:}\\
  {\SEKIPUBLISHEDAS}\par\vspace{\topsep}\noindent
\or
  {\bf The following publication is a short version of this \SEKIREPORTTYPE:}\\
  {\SEKIPUBLISHEDAS}\par\vspace{\topsep}\noindent
\or
  {\bf This \SEKIREPORTTYPE\ refines and extends the following publication:}\\
  {\SEKIPUBLISHEDAS}\par\vspace{\topsep}\noindent
\fi
\ifcase\SEKIREVIEWSTATUS
  {\bf This \SEKIREPORTTYPE\ was edited and the individual contributions were
   sub-edited by:}
  \\\ignorespaces\SEKISUBEDITOR
\or
  {\bf This \SEKIREPORTTYPE\ was internally reviewed by:}
  \\\ignorespaces\SEKIREVIEWER
\or
  {\bf 
   \ifcase\SEKIPUBLISHEDTYPE
      This 
   \or
      This
   \or
      The above short version of this
   \or
      The above previous version of this 
   \fi
   \SEKIREPORTTYPE\ successfully passed the following external 
   anonymous referee process:}
  \\\ignorespaces\SEKIREFEREEPROCESS
\fi
\par\vspace{\topsep}\noindent
{\bf Editor of SEKI series:}\\Claus-Peter Wirth 
\\FR Informatik, Universit\"at des Saarlandes, D--66123 Saarbr\"ucken, Germany
\\E-mail: {\url{cp@ags.uni-sb.de}}
\\WWW: \url{http://www.ags.uni-sb.de/~cp/welcome.html}

\thispagestyle{empty}
\mbox{}}
\cleardoublepage\pagestyle{myheadings}\setcounter{page}{1}}
\catcode`\@=12

\newcommand\robbiuni
% Robbi plus Uni-logo
{\begin{minipage}{6cm}
\vspace*{1.0cm}\par
\hspace{2.55cm}\mbox{\epsfxsize=1cm\epsfysize=1cm\strut\epsffile{seki-eule.eps}}
\vspace*{-6cm}\par
\epsfxsize=5.6cm\epsfysize=10cm
\strut\epsffile{seki-robbi.eps}
\end{minipage}}


\SEKIusersusepackages
\SEKImasterusepackages
\usepackage[T1]{fontenc}
\usepackage{url}
\RequirePackage{epsf}
\usepackage{rotating}

\font\GIGA=cmss12 scaled 4000

\setlength\oddsidemargin{3.0cm}            %intended inner margin
\setlength\textwidth{16.3cm}               %intended textwidth
\setlength\columnsep{1cm}                  %intended columnsepwith in twocolumn
% Remember: dina4 has 21cm breadth
% Thus Your outer margin is 21cm-\oddsidemargin-\textwidth 

\setlength\topmargin{3cm}                  %intended topmargin
\setlength\textheight{24cm}                %intended textheight
% Remember: dina4 has 297mm height
% Thus Your bottom margin is 297mm-\topmargin-\textheight

% Further settings:
\reversemarginpar
\setlength\marginparwidth{1.4cm}
\setlength\marginparsep{0.5cm}
\setlength\parskip{5pt}

% Follows some computation. Please don't modify!
\setlength\evensidemargin{21cm}            %dina4 breadth
\addtolength\evensidemargin{-1\textwidth}  %adjust right
\addtolength\evensidemargin{-1\oddsidemargin}%set margin
\addtolength\evensidemargin{-1in}          %internal correction factor
\addtolength\oddsidemargin{-1in}           %internal correction factor
\addtolength\topmargin{-1in}               %internal correction factor
\addtolength\topmargin{-1cm}               %internal correction factor
\addtolength\evensidemargin{-0.1cm}        %fine tuning

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=11

\def\newtheorem#1{\@ifnextchar[{\@othm{#1}}{\@nthm{#1}}}
 
\def\@nthm#1#2{%
%typical #1=definition, #2=Definition
\@ifnextchar[{\@xnthm{#1}{#2}}{\@ynthm{#1}{#2}}}
 
\def\@xnthm#1#2[#3]#4{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=Definition, #3=section, #4=cpspecial
{\@definecounter{#1}\@addtoreset{#1}{#3}%
\expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
  \csname the#3\endcsname \@thmcountersep \@thmcounter{#1}}%
\global\@namedef{#1}{\@thm{#1}{#2}{#4}}\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@ynthm#1#2#3{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=Definition, #3=cpspecial
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\@thm{#1}{#2}{#3}}\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@othm#1[#2]#3#4{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=theorem, #3=Defintion, #4=cpspecial
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
\global\@namedef{#1}{\@thm{#2}{#3}{#4}}%
\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@thm#1#2#3{\refstepcounter
    {#1}\@ifnextchar[{\@ythm{#1}{#2}{#3}}{\@xthm{#1}{#2}{#3}}}
 
\def\@xthm#1#2#3{\@begintheorem{#2}{\csname the#1\endcsname}{#3}\ignorespaces}
\def\@ythm#1#2#3[#4]{\@opargbegintheorem{#2}{\csname
       the#1\endcsname}{#4}{#3}\ignorespaces}
 
%DEFAULT VALUES
\def\@thmcounter#1{\noexpand\arabic{#1}}
\def\@begintheorem#1#2#3{\trivlist \item[\hskip \labelsep{\bf #1\ #2}]#3}
\def\@opargbegintheorem#1#2#3#4{\trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3)}]#4}
\def\@endtheorem{\endtrivlist}
 
%\def\@thmcountersep{}
%\newtheorem{theorem}            {Theorem}[thmcounter]{\mbox{}\it}
\def\@thmcountersep{.}
\def\globalrequirement{Global Requirement}

\newtheorem{theorem}{Theorem}[section]{\mbox{}\it}
\newtheorem{lemma}     
[theorem]{Lemma}{\mbox{}\it}
\newtheorem{sublemma}  
[theorem]{Sublemma}{\mbox{}\it}
\newtheorem{corollary} 
[theorem]{Corollary}{\mbox{}\it}
\newtheorem{example}   
[theorem]{Example}{\mbox{} \mbox{}\rm}
\newtheorem{remark}    
[theorem]{Remark}{\mbox{} \mbox{}\rm}
\newtheorem{forderung} 
[theorem]{\globalrequirement}{\mbox{}\it}
\newtheorem{requirement} 
[theorem]{Requirement}{\mbox{}\it}
\newtheorem{definition}
[theorem]{Definition}{\mbox{} \mbox{}\rm}
\newtheorem{aufgabe}   
[theorem]{Aufgabe}{\mbox{} \mbox{}\rm}
\newtheorem{specification}
[theorem]{Specification}{\mbox{} \mbox{} \rm}
\catcode`\@=12




